Provable GPU Data-Races in Static Race Detection

We extend the theory behind the Faial tool-chain, which can soundly prove that CUDA programs (aka, kernels) are data-race free using specialized behavioral types called memory access protocols (MAPs). In this paper we extend the theory of MAPs to characterize kernels for which alarms can be identified as true alarms. We introduce a core calculus for CUDA, which we named BabyCUDA, and a behavioral type system for it. We show that if a BabyCUDA program can be assigned a MAP, then any alarm raised by Faial for this program is a true alarm.

==> eptcsdata.tex <==
\providecommand{\firstpage}{36}
\providecommand{\publicationstatus}{M. Carbone and R. Neykova (Eds.): 13th International\\
Workshop on Programming Language Approaches to\\
Concurrency and Communication-cEntric Software\\
EPTCS 356, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.356.4}{10.4204/EPTCS.356.4}}


==> macros-balloon.tex <==
\makeatletter
\newif\iflst@linemark

\lst@AddToHook{EveryLine}{%
  \begingroup
  \advance\c@lstnumber by 1\relax
  \pgfmark{line-\lst@name-\the\c@lstnumber-start}%
  \endgroup
}

\lst@AddToHook{EOL}{\pgfmark{line-\lst@name-\the\c@lstnumber-end}%
\global\lst@linemarktrue
}

\lst@AddToHook{OutputBox}{%
  \iflst@linemark
  \pgfmark{line-\lst@name-\the\c@lstnumber-first}%
  \global\lst@linemarkfalse
  \fi
}

\def\tkzlst@fnum#1\relax#2\@STOP{%
  \def\@test{#2}%
  \ifx\@test\@empty
  \def\tkzlst@start{0}%
  \else
  \@tempcnta=#1\relax
  \advance\@tempcnta by -1\relax
  \def\tkzlst@start{\the\@tempcnta}%
  \fi
}

\lst@AddToHook{Init}{%
  \expandafter\tkzlst@fnum\lst@firstnumber\relax\@STOP
  \pgfmark{line-\lst@name-\tkzlst@start-start}%
}

\newcommand\balloon[4]{%
  \pgfmathtruncatemacro\pgf@temp{%
    #3-1
  }%
  \iftikzmark{line-#2-\pgf@temp-start}{%
    \iftikzmark{line-#2-#3-first}{%
      \xdef\b@lines{({pic cs:line-#2-\pgf@temp-start} -| {pic           cs:line-#2-#3-first})}%
    }{%
      \iftikzmark{line-#2-#3-start}{%
        \xdef\b@lines{({pic cs:line-#2-\pgf@temp-start} -| {pic             cs:line-#2-#3-start})}%
      }{%
        \xdef\b@lines{(pic cs:line-#2-\pgf@temp-start)}%
      }%
    }%
  }{%
    \xdef\b@lines{}%
  }%
  \foreach \k in {#3,...,#4} {%
    \iftikzmark{line-#2-\k-first}{%
      \xdef\b@lines{\b@lines (pic cs:line-#2-\k-first) }
    }{}
    \iftikzmark{line-#2-\k-end}{%
      \xdef\b@lines{\b@lines (pic cs:line-#2-\k-end) }
    }{}
  }%
  \ifx\b@lines\pgfutil@empty
  \else
  \edef\pgf@temp{\noexpand\tikz[remember picture,overlay]\noexpand\node[fit={\b@lines},balloon] (#1) {};}%
\pgf@temp
  \fi
}

\makeatother

\usetikzlibrary{fit,calc,shadows}

% Define styles for balloons, lines and marked code areas
\tikzset{
  line/.style={
    draw,
    rounded corners=2pt,
    -latex
  },
  balloon/.style={
    draw,
    yshift=-3pt,%-2.5pt,
    %fill=yellow!70,
    %dashed,
    opacity=0.2,
    inner sep=0pt,
    rounded corners=4pt
  },
  comment/.style={
    draw,
    fill=yellow!70,
    text=white,
    text width=3cm,
    minimum height=.5cm,
    rounded corners,
    drop shadow,
    align=left,
    font=\footnotesize
  },
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

